Dynamical modelling and origin of gas turbulence in z $\sim$ 4.5 galaxies

In recent years, a growing number of regularly rotating galaxy discs have been found at z $\geq$ 4. Such systems provide us with the unique opportunity to study the properties of dark matter halos at these early epochs, the turbulence within the interstellar medium and the evolution of scaling relations. Here, we investigate the dynamics of four gas discs in galaxies at \textit{z} $\sim$ 4.5 observed with ALMA in the [CII] 158 $\mu$m fine-structure line. We aim to derive the structural properties of the gas, stars and dark matter halos of the galaxies and to study the mechanisms driving the turbulence in high-\textit{z} discs. We decompose the rotation curves into baryonic and dark matter components within the extent of the [CII] discs, i.e. 3 to 5 kpc. Furthermore, we use the gas velocity dispersion profiles as a diagnostic tool for the mechanisms driving the turbulence in the discs. We obtain total stellar, gas and dark matter masses in the ranges of $\log{(M/M_{\odot})} = 10.3 - 11.0$, $9.8 - 11.3$, and $11.2 - 13.3$, respectively. We find dynamical evidence in all four galaxies for the presence of compact stellar components, conceivably stellar bulges. The turbulence present in the galaxies appears to be primarily driven by stellar feedback, negating the necessity for large-scale gravitational instabilities. Finally, we investigate the position of our galaxies in the context of local scaling relations, in particular the stellar-to-halo mass and Tully-Fisher analogue relations.

==> brainstorming.tex <==
%\textcolor{blue}{As discussed in Section~\ref{met:sfr}, we gather photometric data of BRI1335-0417 from the literature to perform SED fitting with \texttt{STARDUST} (see Appendix~\ref{ap:sed} for more details). We find a SFR of XX $\pm$ XX $M_{\odot}$ yr$^{-1}$, which is (or not) consistent with previous reports in the literature, and a stellar mass of $\sim 10^{12} M_{\odot}$, which is more than an order of magnitude above the stellar mass derived with our dynamical modelling, see Appendix~\ref{ap:dynmod} for further discussion.}
%


%These star formation rates were gathered and reported in \citet{romanoliveira23} after being normalised to a Chabrier initial mass function \citep{chabrier03}.
%However, to proceed with a more homogeneous analysis, we use photometric measurements available in the literature to rederive the star formation rates of the galaxies.
%
%For the galaxy BRI1335-0417, a starburst quasar host galaxy, we  choose to rederive the star formation rate by SED fitting. The large SFR of $\sim 5000 M_{\odot}$ reported by \citet{wagg14} and \citet{lu18} might be overestimated due to the contamination of AGN emission in the far infrared.
%
%We gather photometric data from the literature. We summarise all the data available for BRI1335-0417 in Table~\ref{tab:photometry}, ranging from rest-frame UV (887.8 \AA) to rest-frame far-infrared (37.7 mm).
%
%To perform the SED fitting, we employ \texttt{STARDUST} \citep{kokorev21}. The code fits three components independently and simultaneously: stellar, AGN and IR models of dust emission originating from star formation. This is done without the need to assume an energy balance between absorbed UV/optical radiation and the IR emission.
%
%Unfortunately, for the SGP38326 system and J084017 the photometric coverage is not as extensive which hinders the ability to perform the same analysis. Therefore, we limit the SED fitting to only BRI1335-0417.



introduction:




%physical properties of galaxies and function as benchmarks to our understanding of galaxy formation and evolution. The study of these relations under extreme, early universe conditions can further elucidate the physical mechanisms driving the co-evolution of baryons and dark matter in galaxies.

%Recurrent gas accretion and merger events directly induce turbulence \citep{renaud14, elmegreen10, dekel09, forster06}, while other factors, like non-planar or counter-rotating gas streams, are associated with the loss of angular momentum \citep{tacchella16, zolotov15, dekel14}.
%The increase in the ISM turbulence while promoting star formation \citep{parlanti23, ginzburg22, kohandel20, krumholz18}.
%\textit{Moreover, efficient gas accretion can also feed intense star formation associated with intense stellar feedback driven by supernova explosions and stellar winds \citep{ejdetjarn22, orr20, lehnert09}. Active galactic nuclei (AGN) can also promote strong feedback and large scale outflows in galaxies. Both stellar and AGN feedback can increase the turbulence in the ISM through heating and expulsion of gas, balancing the growth of galaxies \citep{nelson19, silk13, hopkins12}.




%\section{Photometric data and SED fitting}\label{ap:sed}
%Following the methodology described in Section~\ref{sec:sfr}, we derive the SFR and stellar mass of the galaxy BRI1335-0417 by fitting its SED with \texttt{STARDUST} \citep{kokorev21}. Since BRI1335-0417 is a quasar host, we also fit the contribution of the AGN to the SED.
%We only fit the rest-frame optical and near-infrared part of the spectrum as there are not enough observations able to constrain the dust component.
%We show the photometric data collected from the literature in Table~\ref{tab:photometry}. The best-fit SFR is XX $\pm$ XX $M_{\odot}$ yr$^{-1}$ and a stellar mass of about $\sim 10^{12} M_{\odot}$. \textcolor{blue}{(comment: I am having trouble reproducing the fit they have with stardust, despite using similar datapoints and the same software. I asked Vasily for some help to settle on a final number.}
%This SFR is consistent \textbf{(or not)} with a recent estimate by \citet{tsukui23} \textbf{(their estimate is 1700 Msun/yr)}, that considers a larger contribution from AGN than other previous values reported in the literature of around $\sim 5000 M_{odot}$ yr$^{-1}$. However, as also noted by \citet{tsukui23}, the stellar mass is higher than the dynamical mass by an order of magnitude, see Appendix~\ref{ap:dynmod} for details. In Figure~\ref{fig:sed}, we show the best-fit SED with the different contributions from stars, AGN and dust.


%\begin{figure}
%    \centering
%    \includegraphics[width=0.48\textwidth]{figures/SED.png}
%    \caption{\texttt{STARDUST} SED fit of BRI1335-0417. The stellar component is shown in blue, the AGN component is shown in green and the dust component is shown in red.}
%    \label{fig:sed}
%\end{figure}



%BRI: William Herschel telescope of the Isaac Newton Group of telescopes in the Canary Islands \citep{storrielombardi96}
%Wagg14: Herschel SPIRE? In Wagg14: S250 mum = 33 ± 6 mJy, S350 mum = 41±5 mJy, and S500 mum = 44±6 mJy}




%\begin{table*}
%    \caption{Photometric data for BRI1335-0417.}
%    \label{tab:photometry}
%    \centering
%        \begin{tabular}{lllll}
%        \hline\hline
%        \multicolumn{5}{c}{BRI1335-0417} \\ \hline
%        \multirow{2}{*}{Instrument/Filter} & Wavelength & Frequency & Flux Density S$_\nu$  & \multirow{2}{*}{Reference} \\
%                          & ($\mu$m)            & (GHz)           & (mJy)    & \\ \hline
%        VLA	            & 203940 & 1.47     & 0.22 $\pm$ 0.04	  & \citet{carilli99}    \\
%        VLA	            & 61685  & 4.86	    & 0.08 $\pm$ 0.01	  & \citet{carilli99}    \\
%        VLA	            & 6813   & 44       & 0.040 $\pm$ 0.007	  & \citet{wagg14}       \\
%        ALMA	        & 2080   & 144      & 1.00 $\pm$ 0.1      & \citet{tsukui23}         \\
%        ALMA	        & 2012   & 149	    & 1.17 $\pm$ 0.07	  & \citet{lu18}         \\
%        IRAM	        & 1350   & 222	    & 5.6 $\pm$ 1.1		  & \citet{guilloteau97} \\
%        IRAM	        & 1250   & 240	    & 10.3 $\pm$ 1.0	  & \citet{omont96}      \\
%        ALMA	        & 1110   & 270	    & 9.03 $\pm$ 0.11	  & \citet{lu18}	     \\
%        ALMA	        & 869    & 345      & 20.5 $\pm$ 2.1	  & \citet{tsukui23}	 \\
%        ALMA	        & 484    & 619      & 52.9 $\pm$ 5.7      & \citet{tsukui23}	 \\
        %SHARC	        & 350    & 857	   & 52 $\pm$ 8		      & \citet{benford99}    \\
%        Spitzer/MIPS$^{1}$    & 24     & 12491    & 1.48 $\pm$ 0.02      & \citet{spitzer21cat}    \\
%        WISE/W4$^{4}$         & 22    & 13571     & 2.82 $\pm$ 0.82       & \citet{cutri14cat}    \\
%        WISE/W3$^{4}$         & 11.56 & 25934     & 0.387 $\pm$ 0.12      & \citet{cutri14cat}    \\
%        Spitzer/IRAC$^{1}$    & 8.0    & 37474    & 0.28 $\pm$ 0.003     & \citet{spitzer21cat}    \\
%        Spitzer/IRAC$^{1}$    & 5.8    & 51688    & 0.151 $\pm$ 0.001    & \citet{spitzer21cat}    \\
%        WISE/W2$^{4}$         & 4.6   & 65172     & 0.116 $\pm$ 0.011     & \citet{cutri14cat}    \\
%        Spitzer/IRAC$^{1}$    & 4.5    & 66621    & 0.1141 $\pm$ 0.0004  & \citet{spitzer21cat}    \\
%        Spitzer/IRAC$^{1}$    & 3.6    & 83276    & 0.1412 $\pm$ 0.0004  & \citet{spitzer21cat}    \\
%        WISE/W1$^{4}$         & 3.35  & 89490     & 0.14 $\pm$ 0.007       & \citet{cutri14cat}    \\
%        VISTA/Ks$^{3}$        & 2.13   & 140500	& 0.102 $\pm$ 0.019	& \citet{mcmahon13, mcmahon19cat}    \\
%        VISTA/H$^{3}$         & 1.63   & 183810   & 0.133 $\pm$ 0.016	& \citet{mcmahon13, mcmahon19cat}    \\
%        VISTA/J$^{3}$         & 1.25   & 240530   & 0.137 $\pm$ 0.01	& \citet{mcmahon13, mcmahon19cat}    \\
%        VISTA/Y$^{3}$         & 1.02   & 294380   & 0.145 $\pm$ 0.01 	& \citet{mcmahon13, mcmahon19cat}    \\
%        SDSS/Z$^{2}$          & 0.90   & 332440   & 0.118 $\pm$ 0.001    & \citet{lasker08, lasker21cat}    \\
%        SDSS/I$^{2}$          & 0.76   & 392660   & 0.102 $\pm$ 0.001    & \citet{lasker08, lasker21cat}    \\
%        SDSS/R$^{2}$          & 0.62   & 479900   & 0.054 $\pm$ 0.001    & \citet{lasker08, lasker21cat}    \\
%        SDSS/G$^{2}$          & 0.48   & 621980   & 0.0099 $\pm$ 0.0003  & \citet{lasker08, lasker21cat}    \\
%        \hline\hline
%        \end{tabular}
%    \begin{tablenotes}
%    \item \textbf{Notes.} $^{1}$ The Spitzer (SEIP) source list (SSTSL2) \citep{spitzer21cat}; $^{2}$ The Guide Star Catalogue \citep{lasker08, lasker21cat}; $^{3}$ The VISTA Hemisphere Survey (VHS) catalog DR4.1 \citep{mcmahon13, mcmahon19cat}; $^{4}$ AllWISE Data Release \citep{cutri14cat}.
%    \end{tablenotes}
%\end{table*}


%Transiting Exoplanet Survey Satellite (TESS) Input Catalog \citep{stassun19, stassun19cat}
%Johnson/V       &   & 541430    & 0.0309 $\pm$ 0.0045 & \citep{stassun19, stassun19cat}


BTFR:


%In this panel, we also show the outer rotation of a subsample of ETGs from the ATLAS$^{\mathrm{3D}}$ survey that have outer low-density HI discs or rings. In this case, the outer rotation velocity we show is measured in the outskirts of the ETGs from the HI emission and we plot the total stellar plus atomic gas mass \citep[purple markers,][]{lelli17}.
%We see that the outer rotation of this sample of ETGs behaves similarly to the flat rotation of disc galaxies \textcolor{red}{probably due to the fact that they both trace the outer gravitational potential.}


%In both panels, we also show elliptical galaxies from the ATLAS$^{\mathrm{3D}}$ survey with circular velocities within 1 $R_{\mathrm{eff}}$ \citep[gray markers,][]{cappellari13}


%The central part of local ETGs  similar way to high-\textit{z} gas discs like the ones in this study.


%Another interesting feature is that local ETGs show two behaviours on both panels:
%\begin{enumerate}
%    \item Outer rotation: on the left panel we show ETGs with outer velocity measurements (purpler markers) that are traced by either rings or diffuse, extended HI emission. These measurements They follow the same trend of spiral galaxies by rotating slower for the same enclosed baryonic mass when compared to ETGs.
%    \item Inner rotation: on the right panel we show the same ETGs with inner velocity measurements that are traced by the stellar rotation. Now, 
%\end{enumerate}

%Likewise, from the SED fit described in Appendix~\ref{ap:sed}, we expect a stellar mass above 10$^{10}$ $M_\odot$, significantly higher than what can be enclosed in the central ring.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.48\textwidth]{figures/tullyfisher_2.pdf}
%    \caption{The baryonic Tully-Fisher relation. We show local disc galaxies in blue \citep{lelli16}, our sample according to the legend and other regular disc galaxies at \textit{z} = 4.5 in magenta \citep{rizzo20, rizzo21}. We show the best-fit for the BTFR at z=0 following the model from \citet{posti19} and the same relation for \textit{z} = 4.5, as described in the text.}\label{fig:btfr2}
%\end{figure}

%Moreover, in Figure~\ref{fig:btfr2} we show our sample of galaxies in addition to the galaxies from \citet{rizzo20} and \citet{rizzo21}, which lie at similar redshift and were analysed in a similar manner. Here, we compare our data not only to the same local spiral galaxies we analysed in Figure~\ref{fig:btfr} \citep[blue points,]{lelli16}, but also the BTFR in the simulations from \citep{torrey14} in the local Universe and at \textit{z}=2 (orange lines).
%
%Moreover, we also show the semi-analytical model for the evolution of the BTFR \citep[black lines,][]{posti19}. The model for the local relation was obtained by fitting the local BTFR with the linear parameters from Table 1 in \citet{posti19}, while the relation at \textit{z} = 4.5 was simply extrapolated from the local BTFR model by changing the cosmological values.


%While in Figure~\ref{fig:btfr} we make an empirical comparison of our sample to other observations to assess the evolution of the baryonic matter and morphology within the galaxies, in Figure~\ref{fig:btfr2} we want to compare our sample to models of disc formation over cosmic time.
%
%We find that the BTFR seems to significantly evolve from \textit{z} $\sim$ 4 in a consistent way with respect to the analytical models and the simulations. This implies that the formation of gas discs over cosmic time are mainly governed by the evolution of the dark matter halo that contains the galaxy. \textbf{does it make sense? should I add more?}





Analysis: the rotation curves were corrected for pressure support, therefore ready to be used in the dynamical modelling; moment 0 maps of the [CII] line and dust emission of the galaxies were obtained and used for modelling the surface brightness profiles; preliminary dynamical models were obtained; the observed velocity dispersions were compared to expected velocity dispersions from models considering different assumptions of turbulence in the galaxies. \\
Still need to: properly obtain errors for the pressure support correction; obtain better fits for the dynamical modelling and settle on the modelling assumptions; obtain better fits of the surface brightness; verify issues with the [CII] moment 0 maps of the galaxies in the galaxy group (due to continuum subtraction issues); properly account for the uncertainties in the dynamical modelling due to the inclination uncertainties; properly measure the [CII] emission and gas masses of the outflow in the centre of one of the galaxies which is a quasar host, possibly extend this analysis to other non-circular regions observed in the other galaxies; obtain star formation rates of the galaxies with SED fitting and compare to the [CII] emission;

dust to gas mass ratio

hst astrometry


Accurate gas dynamics of distant galaxies: resolving the controversies

To this aim, a number of unprecedented observational facilities have been built (e.g. Bacon+ 2010; ALMA partnership 2015) and an impressive theoretical effort has been carried out using sophisticated cosmological hydrodynamical simulations that are run on the World fastest supercomputers (e.g. Schaye+ 2015; Pillepich+ 2018). New detectors and telescopes are capable of observing galaxies at very large distances (high redshift or high-z), which correspond to the earliest epochs of the Universe, when galaxies had just formed. The interpretation of these revolutionary data and thus the possibility to properly constrain models relies on precise measurements. This NWO-funded project will provide this accuracy and precision with the focus on the gas dynamics of high-z galaxies. Galaxy dynamics can be studied by measuring the Doppler shift of gas emission lines across the electromagnetic spectrum. This allows us to determine the amount of rotation at various radii in a galaxy and to estimate the mass of the, otherwise invisible, dark matter (Fig. 1a). Today we can study gas dynamics of very distant galaxies in a similar way at different wavelengths thanks to facilities like the Very Large Telescope (VLT) or the Atacama Large Millimetre Array (ALMA). In fact, one of the most important results of the last decade was that also very distant galaxies are often rotation dominated (e.g. Forster-Schreiber+ 2009; Jones+ 2017). However, distant galaxies are faint and small and determining their rotation curves is not trivial. This project uses a new technique, developed
by the group of F. Fraternali, to overcome these limitations and allow precise measurements back to the very early epochs of galaxy formation. Other than rotation, another property that we will measure precisely is the gas velocity dispersion. This quantifies the turbulence present in the interstellar medium (ISM), which can then be linked to gas accretion, star-formation feedback and the thickness of the gaseous discs (e.g. Glazebrook+ 2013; Wisniowki+ 2015). The amount of rotation in galaxies drives fundamental scaling relations (e.g. Lelli+ 2016, Romanowsky \& Fall 2012) and the determination of their evolution with time is a crucial test for formation models (Fig. 1b).
Fig ure 1.Fig ure 1. a) The rotation curve (circular velocity as a function of radius, points) of the nearby dwarf galaxy WLM (Iorio, Fraternali+ 2017) and mass decomposition with stellar and gas discs (which have minor contribution) and two types of dark matter halos (Read+ 2016). b) Prediction of cosmological hydrodynamical simulations for the Tully-Fisher relation at z=1 (blue points and grey curve) and a comparison with observational data (orange diamonds), from Ferrero+ 2017.
Main goals of the projectMain goals of the project The first goal is to derive rotation and gas velocity dispersions for galaxies at different redshifts from z~1 to z~6 using a homogeneous state-of-the-art methodology. At z=0, rotation curves derived both with neutral hydrogen (HI) (Fig. 1a) and optical emission lines (e.g. Noordermeer+ 2007) have made key contributions to the characterisation of the dark matter (e.g. Navarro+ 1996; Gentile+ 2005; Read+ 2016), the study of the central potentials (de Blok+ 2001) and the importance of stellar feedback (e.g. Pontzen \& Governato 2012). They have had a major impact in the revision of theoretical models to produce more realistic galaxies (e.g. Scannapieco+ 2012; Marinacci+ 2014). However, z=0 is one snapshot of the whole history and going to higher redshift with these studies is of paramount importance.
The second goal is the derivation of the dark matter content in galaxies at these redshifts. To date, there have been only a few pioneering attempts to perform mass decompositions of high-z rotation curves (e.g. Uebler+ 2018) but even the shapes of these curves are a matter of debate (see e.g. Di Teodoro+ 2016 vs Genzel+ 2017). With this project we will obtain reliable mass decompositions of about one hundred high-z galaxies matching, for the first time, the statistics available at z=0.
The third goal is to analyse the resulting scaling relations, in particular the (baryonic) Tully-Fisher (rotation vs baryonic/stellar mass) relation (Tully \& Fisher 1977; McGaugh 2005) and the “Fall” (specific angular momentum j vs stellar mass M*) relation (Fall 1983). From the observational point of view the question whether these relations are evolving with z and how is unanswered. Even at z=1, where the measures are relatively easy to obtain, some groups find that the Tully-Fisher relation is consistent with that at z=0 (e.g. Di Teodoro+ 2016; Harrison+ 2017), while others find that it evolves significantly towards higher velocities and/or lower masses (e.g. Tiley+ 2016; Uebler+ 2017). Thus two major improvements are needed: 1) enlarge the sample, 2) apply the same technique to galaxies at z>1. The study of the Fall relation is fundamental for galaxies because 1) specific angular momentum and mass are independent from each other, 2) they are conserved quantities and 3) one of the most important theories of galaxies formation (the tidal torque theory; Peebles 1969) makes clear and testable predictions. Thus it is a key benchmark for galaxy formation models
(Posti, Fraternali+ 2018) and extending these investigations to higher z is extremely important to distinguish between different scenarios.
This project will also produce accurate velocity dispersions for a large number of galaxies and for different gas tracers including
ionised, neutral and molecular gas. There is a general consensus that gas in high-z galaxies was, on average, more turbulent (higher
velocity dispersion) than in local galaxies. However, quantifying the velocity dispersion has proved challenging and current
measurements show a large spread with very large values that may be affected by observational biases (Fig. 2b). Our software 3D-
Barolo allows us to overcome these biases returning the intrinsic value of the gas velocity dispersion in the disc. This is a key
measure to understand the origin of turbulence (e.g. Krumholz \& Burkhart 2016).
Fig ure 2.Fig ure 2. a) The relation between stellar specific angular momentum (j*) and stellar mass for a sample of galaxy discs at z~1 (squares) compared to
that at z=0 (grey band), from Marasco, Fraternali+ 2019. b) The velocity dispersion of the ionised gas versus redshift for various samples of star-
forming galaxies, from Di Teodoro+ 2016 and Di Teodoro, Grillo, Fraternali+ 2018. The large red circles are obtained with 3D-Barolo.
MethodologyMethodology
During the past years, there has been a revolution in the ways we can study gas dynamics in high-z galaxies. This is thanks to the
development of new optical Integral Field Units (IFUs) such as KMOS and MUSE that allow us to detect gas emission lines (e.g.
Halpha and [OII]) at high z and large millimetre interferometers, in particular ALMA that, allow us to study CO rotational and the [CII]
fine-structure transitions. These data are opening a completely new window on the physics of galaxy formation and changing our
view of the early Universe. Unfortunately, all the kinematic data obtained for high-z galaxies are at low angular resolution, often at
low spectral resolution (typically s>30 km/s for IFUs) and at low signal to noise (S/N) because of the distance.To deal with these data,
the most reliable approach is to model the emission of the galaxy in 3D producing artificial data to compare to the real data (e.g.
Swaters 1999; Josza+ 2007). The group of F. Fraternali has developed the most advanced and most used of such software: 3D-Barolo
(DiTeodoro \& Fraternali 2015). The exploitation of this software at high-z is at the core of my methodology. For details
about the software and its performance see here.
Once the rotation velocity of the gas is determine and corrected for pressure support (Iorio, Fraternali+ 2017), we obtain the circular
speed (goal 1). This is a measure of the gravitation potential and so allows us to infer the distribution of dark matter (goal 2) and
enters the Tully-Fisher relation (goal 3). The last two goals require the use of data at different wavelengths, in particular optical/IR
data for the distribution of the stellar light. These data are available for most of the galaxies that we will study as they are often part
of large programmes, where the fields have been targeted because of the availability of HST imaging. Examples are the COSMOS,
the UDS or the GOODS fields, observed by KMOS and MUSE. Spatially resolved SED fitting or similar techniques will be used to
extract density profiles (DiTeodoro, Grillo, Fraternali+ 2018; Marasco, Fraternali+ 2019). At z>3, excellent data will be available after
the launch of James Webb Space Telescope (JWST).
BibliographyBibliography
ALMA partnership 2015, ApJL, 808L, 3
Bacon, R.; et al. 2010, SPIE, 7735E, 08
de Blok E.; et al. 2001, ApJL, 552, 23
Di Teodoro; E. M. \& Fraternali, F. 2015, MNRAS, 451, 3021
Di Teodoro, E. M.; Fraternali, F.; Miller, S. H. 2016, A\&A, 594, A77
Di Teodoro, E. M.; Grillo, C.; Fraternali, F.; et al. 2018, MNRAS, 476, 804 Fall, S. M. 1983, IAUS, 100, 391
Ferrero, I.; et al. 2017, MNRAS, 464, 4736
Forster Schreiber, N. M.; et al. 2009, ApJ, 706, 1364
Gentile, G.; et al. 2005, ApJL, 634, 145
Genzel, R.; et al. 2017, Nature, 543, 397
Glazebrook, K. 2013, PASA, 30, 56
Harrison, C. M.; et al. 2017, MNRAS, 467, 1965
Iorio, G.; Fraternali F.; et al. 2017, MNRAS, 466, 4159
Krumholz, M. R. \& Burkhart, B. 2016, MNRAS, 458, 1671
Jones, G.; et al. 2017, ApJ, 850, 180
Jozsa, G. I. G.; et al. 2007, A\&A, 468, 731
Lelli, F.; et al. 2016, ApJ, 816, L14
Marasco, A.; Fraternali, F; et al. 2019, A\&A Letters, 621, L6
Marinacci, F.; et al. 2014, MNRAS, 437, 1750
McGaugh, S. S. 2005, ApJ, 632, 859
Navarro, J.; et al. 1996, ApJ, 462, 563
Noordermeer, E.; et al. 2007, MNRAS, 376, 1513
Peebles, P. J. E. 1969, ApJ, 155, 393
Pillepich, A; et al. 2018, MNRAS, 473, 4077
Pontzen, A. \& Governato, F. 2012, MNRAS, 421, 3464
Posti, L.; Fraternali, F.; et al. 2018, A\&A Letters, 612, L6
Read, J. I.; Iorio, G.; Agertz, O. \& Fraternali, F. 2016, MNRAS, 462, 3628
Romanowsky, A. \& Fall S.M. 2012, ApJS, 203, 17
Scannapieco, C.; et al. 2012, MNRAS, 423, 1726
This website uses cookies.
Learn more Got it
Schaye, J., et al. 2015, MNRAS, 446, 521
Swaters, R. A. 1999, Ph.D. thesis, University of Groningen
Tiley, A. L.; 2016, MNRAS, 460, 103
Tully R. B. \& Fisher J. R. 1977, A\&A, 54, 661
Uebler, H.; et al. 2017, ApJ, 842, 121
Uebler, H.; et al. 2018, ApJ, 854, L24
Wisnioski, E.; et al. 2015, ApJ, 799, 209




(galan-de anta 2023) > disc can survive in isolation and they will investigate the effect of mergers




Surface brightness:
Dust data:
BRI and J:
mfs, robust 2, cleaning 3rms, continuum subtracted, uvcontsub removing spw with line, 0.03 arcsec
imfit, rms -1, on image from casa

gas data:
cube, robust 0.5 for bri, 2 for j, cleaning 3rms, continuum subtracted, uvcontsub
immoments mom0, imfit on that

SGP:
no uvcontsub, uvtaper 0.1 arcsec, tclean 1.5rms, imcontsub on cube, creates a continuum and line image. we have a fitorder 0 and fitorder 1, psf from clean cube (no contsub), 0.02 arcsec cell

immoments mom0, imfit





%disc self-gravity (sigma/h = Vr/r)
%genzel08, binner & tremaine 08, davies 11
%mixing of velocities along the line of sight for thick discs
%intrinsic dispersion,or turbulence?
%thermal broadening
%supernova, magnetorotational instability
%drivers of velocity dispersion in hi tamburro09


Thick discs at z $\sim 4.5$
hydrostatic equilibrium
%Given that the average disc inclination of galaxies is 60$^{\circ}$, it is surprising that all galaxies have very low inclinations ($\sim$40$^{\circ}$) when the disc thickness is not taken into account. This can indicate that it is not appropriate to neglect disc thickness for these galaxies. Moreover, if the galaxies are as thick as the order of a kpc, then they are in a regime similar to the thickest mocks we tested in Section~\ref{sec:CANNUBI}. The intrinsic values of inclination and thickness for those were successfully retrieved with \texttt{CANNUBI} with the minimisation in the full cube, which is the procedure we used for the real galaxies so we consider these values reliable.

Finally, we compared the retrieved disc thickness to theoretical estimations. In order to do so, we considered that the potential well of the galaxies in our sample is dominated by their gas content, such that we can estimate the thickness of the disc as the thickness of the gas layer in hydrostatic equilibrium. A self-gravitating layer has a vertical distribution that follows an $\sech^2$ distributon \citep{vanderkruit81}, which can be written as:

\begin{equation}\label{eq:he1}
    h = \frac{\sigma}{\sqrt{2 \pi G \rho_0}} 
\end{equation}

Where $h$ is the disc scale height, $\sigma$ is the velocity dispersion, $G$ is the gravitational constant and $\rho_0$ is the mid-plane gas density. In the case of disc galaxies we measure the gas surface density $\Sigma$ which can be related to the density in the mid-plane by:

\begin{equation}\label{eq:he2}
    \rho_0 = \frac{\Sigma}{2 h}
\end{equation}

Using Eq.~\ref{eq:he2} and Eq.~\ref{eq:he1} we find that the theoretical thickness $h$ can be obtained with:

\begin{equation}\label{eq:he}
    h = \frac{\sigma^2}{\pi G \Sigma}
\end{equation}

For $\sigma$ we use the mean velocity dispersion ($\sigma_{\textrm{m}}$) reported in Table~\ref{tab:vel}. For $\Sigma$, we can assume that the [CII] distribution is a good tracer of the cold gas profile and that the molecular gas mass is dominant \citep{tacconi18}. So we derive an estimation of the gas surface density in the same radial range as the external velocities by renormalising the [CII] surface brightness profile given by \texttt{$^{\text{3D}}$BAROLO} with the total molecular gas masses from Table~\ref{tab:masses}. 

The assumption of self-gravity of the gas in hydrostatic equilibrium depends on the galaxies being gas dominated. Since we have no information of the stellar component this could be untrue for some of the galaxies, therefore, these results should be interpreted with caution. The only galaxy in our sample with a literature estimate of the stellar mass is AzTEC1, which we are not running this analysis. That being said, the estimated disc scale heights are: 1.3, 1.1, 1.1 and 0.1.

We find that for BRI1335-0417 the values are consistent with each other within a 2$\sigma$ interval. In \citet{tsukui21}, a dynamical modelling of BRI1335-0417 showed that the disc mass is very similar to the total gas mass, indicating that the assumption of gas-only hydrostatic equilibrium can be sufficient. For J081740, SGP38326-1 and SGP38326-2 the measured disc thickness is significantly larger than the one predicted and likely we need to take into account the stellar component as well.

%For comparison, in \citep{walter22} estimates a disc thickness of the order of 100pc for a z $\sim$ 7 quasar.


Firstly, it has been long shown that for galaxy discs to remain globally stable over long periods of time they need to be hosted by a massive spherical component such as a cold dark matter (CDM) halo \citep{ostriker73}. Although, a Navarro-Frenk-White (NFW) CDM halos have low concentrations at high-\textit{z}, which means that massive high-\textit{z} galaxies can be strongly baryon dominated in the inner regions that can be probed with current instruments.
Secondly, massive and low turbulence discs can also become locally unstable due to their own self-gravity \citep{toomre64}.
Lastly, discs are fragile structures that can be easily destroyed during merger events. 
Moreover, the need for massive spherical components, such as cold dark matter halos, to ensure the stability of galaxy discs poses additional difficulties, as high-\textit{z} halos have low concentrations.
%discs take a long time to form: Feng et al. 2015; Zavala et al. 2016; Dubois et al. 2016; Pillepich et al. 2018

%We also investigate the role of turbulence in shaping the properties of galaxies at redshift 4.5, shedding light on the complex physical processes that govern the ISM of galaxies in the early universe.

 %Moreover, the velocity dispersion shows a downtrend profile similar to galaxies in the Local Universe. This suggests that the common assumption at high-\textit{z} of constant velocity dispersion across the disc is not valid. Moreover, it implies that the mechanisms responsible for the turbulence may be stronger in the centre of the galaxies. For the case of BRI1335-0417, a quasar host, this may be due to an central outflow from the supermassive black hole.

%reliability, hydro eq. calculation, do we believe it or not, low s/n in the outer parts (which is used to determine the thickness), no constant thickness -- no clear what we are measuring and $h$, the theoretical disc thickness assuming a gas dominated disc in hydrostatic equilibrium.
%\textcolor{red}{all cube vs. total map
%minor mergers driving the thickness?
%\textbf{alpha cii to justify the thicknspotiess we get?}
%flaring -- what does CANNUBI recover as thickness?
%hydrodynamical equilibrium values here
%THICKNESS: puffed galaxies, form thick, what happens afterwards}
%1) low S/N data, the signal we are trying to measure is faint and it can be due to something else entirely, outflows? Accretion? Distortions?
%2) we are assuming constant thickness across the disc! What do we measure then? Maybe the outer ring 
%3) Hydro eq. is extremely simplified, almost embarrassingly so: we use only the gas with very uncertain mass, no gas distribution, constant thickness again, constant dispersion…!




%
The stellar masses of the galaxies in our sample are likely in between M$_{*} = 10^{10} - 10^{11}$M$_\odot$ and only BRI1335-04217 and J081740 have V$_{\mathrm{rot}} \sim $ 200 km s$^{-1}$. However, given the trending decline of the V/$\sigma$ up to \textit{z} = 3, we expect a median V/$\sigma$ not higher than 4 for TNG50 massive galaxies.
%
Therefore, the diverse population of galaxies we analyse in this study and the extended sample, which were selected only for high-resolution data, have rotation dominated discs not systematically found in those simulations.
Such discrepancy is even worsened if we consider that the galaxies in our sample hav SFR typically higher than the ones from simulations and, therefore, are expected to have higher turbulent motions (i.e., $\sigma \geq$ 100 km s$^{-1}$).


\subsubsection{Toomre Stability Criterion}

To analyse the local stability in the gas disc we compute the Toomre Q parameter as described in Section~\ref{sec:met_q}. In Figure~\ref{fig:Q}, we show the Toomre Q parameter, in logscale, across the galactic radius of the galaxies in our sample. Within the errors, the four galaxies are consistent with a marginally unstable disc (Q $\approx$ 1), with a more stable disc in the inner regions (Q > 1) which could be due to the generally higher velocity dispersions measured closer to the centre.

we should say more about the individual galaxies and discussing the two SGPs, which are nominally below 1 although compatible at 1 sigma, what can the reasons be? what do they have different from the others?

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/toomreq.pdf}
    \caption{Log Toomre Q parameter across galactic radii.}
    \label{fig:Q}
\end{figure}

%\citep{blandhawthorn23} -> stellar bars happen quickly in the centre of baryon dominated disc galaxies

%\textbf{mention recent results obtained with JWST about the presence of stellar bars up to very high-z + theoretical models that say that the bar can form only in dynamically cold disks}


\textbf{Toomre Q (Aditya 2023), stability, limits of Q gas, 2D, stellar component not included, https://arxiv.org/pdf/2304.07734.pdf, https://arxiv.org/pdf/2303.13858.pdf}


radial motions -- sgp?

-> hubble camera title in figures, is it correct?

check SED, SFR


SGP:

**Oteo+2016 -- https://ui.adsabs.harvard.edu/abs/2016ApJ...827...34O/abstract

Riechers+2017 -- https://ui.adsabs.harvard.edu/abs/2017ApJ...850....1R/abstract
Ivison+2016 - https://ui.adsabs.harvard.edu/abs/2016ApJ...832...78I/abstract
Stacey+2021 -- https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.3667S/abstract



J0817:

Neeleman+2017 -- https://ui.adsabs.harvard.edu/abs/2017Sci...355.1285N/abstract
Jones+2017 -- https://ui.adsabs.harvard.edu/abs/2017ApJ...850..180J/abstract
**Neeleman+2020 -- https://ui.adsabs.harvard.edu/abs/2020Natur.581..269N/abstract
Wenkai+2019 -- https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.1619H/abstract
Lagache+2018 -- https://ui.adsabs.harvard.edu/abs/2018A%26A...609A.130L/abstract




In the past decade, our understanding of high-redshift galaxies has changed dramatically with the discovery of numerous cold discs much earlier in the Universe than previously expected. Within the theoretical background of galaxy formation, galaxies are expected to grow hierarchically by accreting gas from intergalactic medium (IGM) and merging with other galaxies throughout cosmic time \textbf{CITE}. Galactic growth is also constantly regulated by feedback processes from either supernovae feedback or active galactic nuclei (AGNs) that warm and eject gas \textbf{CITE}. \textbf{Within this violent context, it was surprising to discover that galaxies are much less turbulent than our predictions...}

\textbf{i) Recent observations of cold discs at high-z and how it impacts the field. \citep{neeleman20} \citep{rizzo20} \citep{fraternali21} \citep{lelli21} }

\textbf{ii) simulations, Kretschmer et al. submitted}

\textbf{iii) amazing data with ALMA, [CII] emission (tracer of atomic/molecular gas), carefully modelling taking into account limitations of the observations, new view of the high z universe even at low SNR and low angular resolution}

\textbf{iv) submm galaxies, infrared, HST (restframe far UV), JWST}


%As you know, the main difference with respect to Galpak is that it is non-parametric. I think that this is an advantage but in some cases a parametric fit is also useful as it is global and not ring by ring. Galpak then could have the advantage that it uses MCMC but obviously in these galaxies there is no need, we can simply use SPACEPAR in BB and that removes any problem on possible dependence on initial guesses. I think that this should be stressed in our paper, in my I even put the outputs of SPACEPAR.. Then if they ask me I would say that BB is the culmination of decades of 3D kinematic experience of the HI community. In this sense it employs a solid methodology and also because of this it provides all the outputs and checks that you need to judge your fit. It is completely not a black box, quite the opposite. But some people appreciate this more than others.








investigate the radial motions -- anything new from Tadaki+2020? higher dispersion?


Hst astrometric calibration (gabe from DAWN)


Iorio+2017
Mancera pina + 2020
Read 2016
Mancera pina 2022


Discussion:


bar in SGP? dust...
bar: efstathiou+82 criterion for bar stability (see A1 in bland-hawthorn+23, check fdisk?)

comparison between escape velocity and outflow velocity

global and inner region

Hopkins+17 -> outflow/turbulence


outflow fraction in gas rich galaxies -> eta vs. stellar mass
Pandya+22

Hopkins+23
deep potential: outflows are suppressed, star formation is steady, disc is formed

escape velocity plays an important role

disc stability with respect to the DM halo (or bulge halo)


turbulence vs. radius -> not constant, different or stronger mechanisms
dust -> star formation
SFR (dust model) vs. turbulence (spatially resolved)

Toomre Q
dynamical timescales
no krumholz model (Q2d makes no sense)


outflows:
daniel mcpherson
Bron Reichardt Chu 22a,b
chelsea sharon
arianna lang -> discs jwst
agn feedback in co: chelsea sharon


disc thickness:
thick discs are old and high dispersion
thick discs are alpha rich, thin discs are alpha poor
alpha rich -> SNII core collapse (immediate)
alpha poor -> SNIa -> takes longer to enrich
origin: Kloperskov 22 bursty accretion, clarke19



baryonic tully fisher relation: Vcirc, baryonic mass (stars+gas), di teodoro 2016
fall relation: gas mass and angular momentum, posti 2018, 2016, mancera pina etc
angular momentum: r, vrot, surface brightness

mass size relation
mass vs v/sigma


Check: Ana's paper physics

Understand:
what is lyman alpha emission
lyman and Balmer break (which one is the 4000 angstrom)

Check possible papers that are out:
Uebler as first author and as not first author

Parlanti (with Halpha for Lelli's galaxy)





written passages:






check on paper: alpha cii, sfr cii, sfr from dust (resolved)
gas to dust ratio

cii flux comparison with low resolution data, total gas mass

sfr:
kennicutt, cecilia
cii sfr
cii -> alphacii
sed fitting

Hi Fernanda, thank you so much.There's three papers I found interesting on this topic : Zanella+18 where they introduced the [CII]-based molecular gas mass calibrations, Dessauges-Zavadsky+20 : they compare the [CII] based molecular gas masses for high-z  main-sequence DSFGs and Vizgan+22 : They use galaxies from the SIMBA simulation (if im not wrong, but it's on simulations) and compare [CII] as molecular gas tracer and SFR tracer.

There are some more theoretical works on [CII] as molecular gas tracer Sommovigo+21, which is also super interesting





mass loading factor


Discussion

evolution over cosmic time (tully fisher)


Results mass modelling:
DM halo, constraints on stellar mass and radius, precise determination of gas mass
Alpha CII?


Dynamical timescale of the discs, CII is a better tracer of sfr or gas mass?


turbulence
	krumholz
	SN energy

outflows
	mass load factor

dynamical mass vs dispersion

depletion time for cold gas

toomre q gas -> stability (marinacci)
	as a function of radius
	globally unstable?
	creation of an spheroidal component?
	genzel+2014


\subsection{Photometric data}

astrometric calibration for the uv data with hubble

Estimating stellar mass: SED, main sequence


\subsection{SED fitting with Lephare}

\subsection{Error in the inclination}

\subsection{Galfit}
galfit fit to dust



imfit / visibility plane for fitting the dust/gas (sweden, tool)


gas to dust, alpha cii, alpha co (if converges, then fix)


fit stellar mass and halo mass with flat prior


 However, the presence or absence of a velocity gradient does not confirm nor deny the dynamical state of a galaxy, a comprehensive 3D analysis of the emission is necessary to distinguish discs and mergers \citep{rizzo21}.


mass outflow rates -- kade, kiana 22



\subsection{Local stability in the disc}\label{sec:met_q}

To estimate the local instabilities in the gas disc, we calculate the Toomre Q parameter using the standard definition,
%
\begin{equation}
    Q(R) = \frac{\kappa \sigma}{\pi G \Sigma_{\mathrm{gas}}},
\end{equation}
%
where $\kappa$ is the epicycle frequency, i.e. the oscillation frequency of the radial perturbation of a test particle within an axisymmetric potential \citep{toomre64}. This is defined as
%
\begin{equation}
    \kappa = \sqrt{R \frac{d\Omega^2}{d R} + 4 \Omega^2},
\end{equation}
%
where $\Omega$ is the angular frequency ($\Omega = V_{\mathrm{rot}}/R$).

When the value of Q is approximately 1, then portions of the disc can become marginally unstable and collapse under their own gravity, potentially leading to star formation \citep{ginzburg22, kohandel20, krumholz18}. If Q is higher than 1 then the disc is stable against local instabilities, likewise, if Q is lower then the disc is unstable.


scaling relations
	stellar to halo mass
	SFR vs stellar mass
	tully fishers
	angular momentum


CII SFR



\begin{enumerate}
	\item table with gas mass, stellar mass, halo mass
	\item depletion time for cold gas + SFR
	\item Dynamical mass vs dispersion
	\item Tully Fisher (what kind of tully fisher, what kind of progenitors are they?)
	\item Stellar to halo mass
	\item SFR vs stellar mass
\end{enumerate}

Q parameter

alpha cii


SFR relation Capak+15 CII/SFR

gravity - filippo's equation

